Dreams Are More "Predictable'' Than You Think

A consistent body of evidence suggests that dream reports significantly vary from other types of textual transcripts with respect to semantic content. Furthermore, it appears to be a widespread belief in the dream/sleep research community that dream reports constitute rather ``unique'' strings of text. This might be a notable issue for the growing amount of approaches using natural language processing (NLP) tools to automatically analyse dream reports, as they largely rely on neural models trained on non-dream corpora scraped from the web. In this work, I will adopt state-of-the-art (SotA) large language models (LLMs), to study if and how dream reports deviate from other human-generated text strings, such as Wikipedia. Results show that, taken as a whole, DreamBank does not deviate from Wikipedia. Moreover, on average, single dream reports are significantly more predictable than Wikipedia articles. Preliminary evidence suggests that word count, gender, and visual impairment can significantly shape how predictable a dream report can appear to the model.

==> _images/wk_db_bertb_pca_kmc.tex <==

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\columnwidth]{./_images/wk_db_bertb_pca_kmc.pdf}
    \caption{\label{fig:wk_db_bertb_pca_kmc.pdf} Report and article space. PCA visualisation of the embedding space of DreamBank's reports and WikiText2's articles. Style and size indicate the cluster identified by the unsupervised KM clustering algorithm.}
\end{figure}

==> _tables/ppl_stats.tex <==

\begin{table}[htb!]
\centering
\resizebox{.6\columnwidth}{!}{%
\begin{tabular}{lc}
\hlineB{3}
\textbf{Statistic} &    \textbf{Value} \\
\hlineB{3}
Count &           21607 \\
Mean  &              49.55 \\
Standard deviation   &             401.78 \\
min   &               4.42 \\
25\%  percentiles  &              25.19 \\
50\% percentiles  &              32.67 \\
75\% percentiles  &              45.74 \\
max   &           56966.58 \\
\hlineB{3}
\end{tabular}
}
\caption{\label{tab:pplx_stats} Statistics of the collected perplexoty scores.}
\end{table}
